Accelerating Retrieval-Augmented Generation

An evolving solution to address hallucination and enhance accuracy in large language models (LLMs) is Retrieval-Augmented Generation (RAG), which involves augmenting LLMs with information retrieved from an external knowledge source, such as the web. This paper profiles several RAG execution pipelines and demystifies the complex interplay between their retrieval and generation phases. We demonstrate that while exact retrieval schemes are expensive, they can reduce inference time compared to approximate retrieval variants because an exact retrieval model can send a smaller but more accurate list of documents to the generative model while maintaining the same end-to-end accuracy. This observation motivates the acceleration of the exact nearest neighbor search for RAG. In this work, we design Intelligent Knowledge Store (IKS), a type-2 CXL device that implements a scale-out near-memory acceleration architecture with a novel cache-coherent interface between the host CPU and near-memory accelerators. IKS offers 13.4-27.9x faster exact nearest neighbor search over a 512GB vector database compared with executing the search on Intel Sapphire Rapids CPUs. This higher search performance translates to 1.7-26.3x lower end-to-end inference time for representative RAG applications. IKS is inherently a memory expander; its internal DRAM can be disaggregated and used for other applications running on the server to prevent DRAM, which is the most expensive component in today's servers, from being stranded.

==> Figures/5-Architecture/iks-overview-backup.tex <==
\begin{figure*}[!ht]
    \centering 
    
    \begin{subfigure}[b]{0.2\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/IKS_V1.pdf}
        \caption*{\textbf{(b)}}
        \label{fig:iks_structure:iks-v1}
    \end{subfigure}
    \begin{subfigure}[b]{0.35\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/NMA_V1.pdf}
        \caption*{\textbf{(c)}}
        \label{fig:iks_structure:nma-v1}
    \end{subfigure} 
    \begin{subfigure}[b]{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/DPU_V1.pdf}
        \caption*{\textbf{(d)}}
        \label{fig:iks_structure:dpu-v1}
    \end{subfigure}
    \begin{subfigure}[b]{0.15\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/TKU_V1.pdf}
        \caption*{\textbf{(e)}}
        \label{fig:iks_structure:tku-v1}
    \end{subfigure}

    \caption{(a) IKS includes eight LPDDR5X packages with one near-memory accelerator (NMA) chip near each package. (b) IKS internal DRAM, scratchpad spaces, and configuration registers are mapped to the host address space. The scratchpad and configuration register address ranges are labeled as \textit{Context Buffers}. (c) Each NMA includes 64 processing engines. (d) Each dot-product unit includes 68 MAC units. (e) Top-K unit and Top-K scratchpad structure.}
    \label{fig:iks_structure}
\end{figure*}
\begin{comment}
\begin{figure*}[!ht]
    \centering 
    
    \begin{subfigure}[b]{0.2\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/IKS_V1.pdf}
        \caption*{\textbf{(b)}}
        \label{fig:iks_structure:iks-v1}
    \end{subfigure}
    \begin{subfigure}[b]{0.35\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/NMA_V1.pdf}
        \caption*{\textbf{(c)}}
        \label{fig:iks_structure:nma-v1}
    \end{subfigure} 
    \begin{subfigure}[b]{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/DPU_V1.pdf}
        \caption*{\textbf{(d)}}
        \label{fig:iks_structure:dpu-v1}
    \end{subfigure}
    \begin{subfigure}[b]{0.15\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/TKU_V1.pdf}
        \caption*{\textbf{(e)}}
        \label{fig:iks_structure:tku-v1}
    \end{subfigure}

    \caption{(a) IKS includes eight LPDDR5X packages with one near-memory accelerator (NMA) chip near each package. (b) IKS internal DRAM, scratchpad spaces, and configuration registers are mapped to the host address space. The scratchpad and configuration register address ranges are labeled as \textit{Context Buffers}. (c) Each NMA includes 64 processing engines. (d) Each dot-product unit includes 68 MAC units. (e) Top-K unit and Top-K scratchpad structure.}
    \label{fig:iks_structure}
\end{figure*}
\end{comment}

==> Figures/5-Architecture/nma-arch.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.3\linewidth]{Figures/NMA_V1.pdf}
    \caption{NMA architecture.}
    \label{fig:nma-arch}
    \vspace{-5pt}
\end{figure}


==> Figures/5-Architecture/top-knn.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{Figures/NMA_MF.pdf}
    \caption{Top-K Selection Unit.}
    \label{fig:top-knn}
    \vspace{-15pt}
\end{figure}

==> Figures/Experimental_Results/Mistral-Time-To-Interactive.tex <==
\begin{figure}[t]
\centering
    \centering


\includegraphics[width=.8\linewidth]{Figures/Experimental_Results/Time-To-Interactive-CPURetrieval-4.png}
\caption{Breakdown of time-to-interactive latency for QA RAG applications, large models for various passage counts. Retrieval on CPU, over large QA corpus. \derrick{generating this with K=32 for Mistral as well.}
    }
    \label{fig:Mistral-LLama-TTI}

\label{fig:generation-accel}
\end{figure}


==> Figures/Introduction/float-overview.tex <==
\begin{figure*}[htbp]
    \centering
    \begin{subfigure}[b]{0.14\textwidth}
        \includegraphics[width=\textwidth]{Figures/Introduction/overview-baseine}
        \caption{Baseline CPU}
        \label{fig:overview:baseline}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.21\textwidth}
        \includegraphics[width=\textwidth]{Figures/Introduction/overview-pcie}
        \caption{PCIe Accelerator}
        \label{fig:overview:pcie}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.14\textwidth}
        \includegraphics[width=\textwidth]{Figures/Introduction/overview-shared}
        \caption{Shared on-chip}
        \label{fig:overview:shared}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.14\textwidth}
        \includegraphics[width=\textwidth]{Figures/Introduction/overview-private}
        \caption{Private on-chip}
        \label{fig:overview:private}
    \end{subfigure}
    \hfill
        \begin{subfigure}[b]{0.14\textwidth}
        \includegraphics[width=\textwidth]{Figures/Introduction/overview-cdcore}
        \caption{\arch (proposal)}
        \label{fig:overview:cdcore}
    \end{subfigure}
    
    \caption{Computing landscape of performing compression and decompression.}
    \label{rfidtag_testing}
\end{figure*}





==> Figures/Motivation/SiliconEfficiency.tex <==
\begin{figure}[b]
  \begin{center}
    %\vspace{-15pt}
    \includegraphics[width=0.45\textwidth]{Figures/Motivation/images/Silicon-Efficiency.png}
  \end{center}
  \vspace{-10pt}
  \caption{Relative performance density (throughput per area) of various CPUs running \cd on inputs representative of hyperscaler workloads.\malian{Update the figure using the "Core + L2 + LLC Area" in Table 2 and new throughput numbers}}
  \label{fig:silicon-efficiency}
  
  \vspace{-10pt}
\end{figure}


==> Figures/Motivation/ann-acc-fid.tex <==
\begin{figure}
    \centering

    \includegraphics[width=0.8\linewidth,trim=5cm 7cm 3cm 6cm]{Figures/Profiling/ann_acc_fidt5.pdf}
        \caption{Accuracy score (recall) for \appt, equipped with \enns and \anns for various document counts (K). %For \appl, recall scores could not be gathered for $K=32$, as the sequence length exceeded the model's maximum sequence length of 4096 tokens.
       }
        \label{fig:ann-acc-t5}
    
\end{figure}

==> Figures/Motivation/ann-acc-llm.tex <==
\begin{figure}

    \centering
    \begin{subfigure}[b]{0.4\textwidth}
     \centering

    \includegraphics[width=\textwidth]{Figures/Profiling/ann_acc_fid.pdf}
        \caption{\appt.}
        \label{fig:ann-acc-t5}
            \end{subfigure}


    \begin{subfigure}[b]{0.4\textwidth}
             \centering


    \includegraphics[width=\textwidth]{Figures/Profiling/ann_acc_llm.pdf}
        \caption{\appm and \appl.
       }
        \label{fig:ann-acc-llm}

        \end{subfigure}

    \caption{Accuracy scores (recall) vs. document count (K) for all pipelines. 
    }
    \label{fig:ann-acc}
\end{figure}

==> Figures/Motivation/latency_k.tex <==
\begin{figure}

    \centering

    

    \includegraphics[width=.5\textwidth]{Figures/Motivation/ksensitivity.pdf}


    \caption{Latency breakdown of \appt, \appm, \appl for various values of K, 50 GB corpus, and batch size 1. Retrieval is \enns and runs on CPU, generation runs on a single Nvidia A100 for \appt and \appm, and 2 A100s for \appl. 
    }
    \label{fig:ksensitivity}
\end{figure}

==> Figures/Motivation/llm-end-to-end.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figures/Experimental Results/llm-breakdown.pdf}
    %\caption{Accelerated retrieval performance. An optimized GEMM implementation, making optimal use of the cache hierarchy in conjunction with SIMD operations (e.g., Intel's MKL BLAS implementation using AVX-512), can perform search faster than Intel's AMX-accelerator for smaller batch sizes. As the batch size increases, search shifts from memory- to compute- bound, eventually causing AMX to reduce search times below what is achievable in BLAS-MKL. }
    %\caption{Accelerated Retrieval Performance. Shows how optimized GEMM with cache optimization and SIMD (e.g., Intel's MKL BLAS using AVX-512) outperforms Intel's AMX for small batch sizes. As batch size grows, the task becomes compute-bound, allowing AMX to surpass BLAS-MKL in search speed.}
    \caption{Breakdown of end-to-end generation time for \appl and \appm. Retrieval runs on the CPU for 50 GB and 512GB corpus sizes. X-axis is the value of K.}
    \label{fig:llm-end-to-end}
\end{figure}

==> Figures/Profiling/ann-acc-llm.tex <==
\begin{figure}
    \centering

    \includegraphics[width=0.8\linewidth]{Figures/Background/ann_acc_llm.pdf}
        \caption{Accuracy score (recall) for \appm and \appl, equipped with \enns and \anns for various document counts (K). %For \appl, recall scores could not be gathered for $K=32$, as the sequence length exceeded the model's maximum sequence length of 4096 tokens.
       }
        \label{fig:ann-acc-llm}
    %\globaltrim
    
\end{figure}

==> Figures/Profiling/retrieval_platforms.tex <==

\begin{table}
    \centering
    \begin{tabular}{c|cccc}
        Batch Size & \multicolumn{2}{c}{1} & \multicolumn{2}{c}{16}\\
         Corpus Size& 50  & 512 & 50 & 512 \\
        \hline 

         CPU& 1  & 1 & 1 & 1\\
         AMX& 1.05 & 1.10 & 1.59 & 1.70\\
        GPU & 8.6 & 37.1 & 31.7 & 201\\

    \end{tabular}
    \caption{Speedup of AMX and GPU for \enns, relative to a CPU baseline. AMX speedup is flat for very small batch sizes. For 50GB and 512GB corpus size, 2 and 13 A100 GPUs are used, respectively. GPU speedups assume linear performance scaling.}
    \label{tab:retrieval_platforms}

    \globaltrim


\end{table}

==> Figures/Tables/AcceleratorAreaComparisons.tex <==
\begin{table}[b]
\centering
\caption{Resource utilization of monolithic (De)Compression Accelerators. We use the 64kB window size ZSTD Configuration for \cite{karandikar2023cdpu}. \cite{abali-2020-nxu} and ~\cite{fowers_scalable_2015} target the Deflate~\cite{deflate} compression algorithm.}
\label{tab:res}
\begin{tabular}{|c|c|c|}
\hline
Accel & Resources/Area & Bandwidth \\ \hline
IBM's z15 (De)Compressor~\cite{abali-2020-nxu}  & 0.05\% chip area & 15GB/s  \\ \hline
Parallel Deflate FPGA~\cite{fowers_scalable_2015}  & 39078 ALMs    &  2.7 GB/s \\ \hline
ZSTD CDPU~\cite{karandikar2023cdpu} & 1.9 mm2 in 16nm & 3.95 GB/s \\ \hline
\end{tabular}
\end{table}



==> Figures/Tables/DCU_Resource_Utilization.tex <==
\begin{table}[b]
\centering
\caption{Resource utilization of \unit{s}. General purpose lossless compression components are reused from ~\cite{karandikar2023cdpu}. }
\label{tab:res}
\begin{tabular}{|c|c|c|}
\hline
\unit & Resources(LUTs) & Figure Of Merit (Ops/Sec, Bandwidth, etc.)\\ \hline
HuffmanCompressor~\cite{karandikar2023cdpu}  & & \\ \hline
LZ77MatchFinder~\cite{karandikar2023cdpu} & &  \\ \hline

 & 1.9 mm2 in 16nm & 3.95 GB/s \\ \hline
\end{tabular}
\end{table}

==> Figures/Tables/cpu-iks-gpu.tex <==
\begin{table}
    \smalltable
    \centering
    \begin{tabular}{c|cccccccccc}
         Corpus Size & \multicolumn{2}{c}{50 GB}  & 
         \multicolumn{2}{c}{\edit{200 GB}} &
         \multicolumn{2}{c}{512 GB} &
         \multicolumn{2}{c}{1 TB} &
         \multicolumn{2}{c}{2 TB}\\
         Batch Size &  1  &  16&1  &16 & 1  &16 & 1 & 16 & 1 & 16\\
         \hline

         CPU (s) & 0.85 & 2.4 & 3.4 &  9.6 & 8.7  & 24.6 & 17.4 & 49.2 & 34.8 & 98.4 \\
         AMX (s) & 0.81 & 2.3 & 3.1& 9.2& 8.0 & 22.6 & 16.0 & 45.2 & 31.9 & 90.2 \\
         
         GPU (ms) & 120.2 & 210.4  & 166.3 & 287.8 & 185.6& 326.0& N/A & N/A & N/A & N/A  \\
         1 IKS (ms) & 46.0 & 46.1 & 183.8 & 183.9 & 470.6 & 470.7 & N/A & N/A& N/A & N/A\\
         4 IKS (ms) & 11.5 & 12.0 & 46.0 & 47.9 & 117.7 & 118.2 & 229.8 & 230.4 & 459.6 & 460.2 \\
    \end{tabular}
    \caption{Comparison of \enns retrieval time (in milliseconds): CPU, AMX, GPU, IKS, in various configurations. \editlow{GPU } \derrick{ "We will extend Table-3 to also include results for weak scaling and add a scalability discussion in the draft."}\malian{what is the methodology for 7GPU results? Is this extrapolation or real runs?}\derrick{Extrapolation, we mention the methodology in table 1.}\malian{Shouldn't you add rows for larger corpos sizes to this table to show scalability?} \derrick{Do one line of GPU (plus another for time to copy the corpus), run on real if possible for 8x. Add 1 TB and 2 TB}}
    \label{tab:CPU-IKS-GPU}
    \vspace{-15pt}
\end{table}

==> Figures/Tables/power_area_IKS.tex <==
\begin{table}
\smalltable
    \centering
    \begin{tabular}{c|cccc}
        Corpus Size & \multicolumn{2}{c}{50 GB} & \multicolumn{2}{c}{512 GB} \\
         
          &    &   &  & \\
         \hline
         &  &  &  & \\
         
          & &  &  &  \\
         
          &  &  &  &  \\
          &  &  &  &  \\

         \hline
          &  &  &  &  \\
    \end{tabular}
    \caption{Power and Area Comparison\derrick{Pending finalized area figures}}
    \label{}
\end{table}


==> Methodology.tex <==
\section{Methodology}
\label{sec::Methodology}
We model groups of between 1-8 CDCores using gem5. The cores are modelled after ARM N1 neoverse cores, with the key difference being the hardware modifications outlined in the previous section.

\noindent\textbf{Workloads.} We compare CDCores' performance with unmodified neoverse cores using a set of microbenchmarks developed to represent datacenter (de)compression use cases.

\noindent\textit{Fast Database Decompression} We construct a workload involving decompressing a 4kB-128kB block, indexing into it, performing an operation and returning it. This idiom represents the sequence of steps that would occur when performing an operation like a MERGE on two items stored within a row-oriented database.

\noindent\textit{Fast RPC (De)compression} To emulate swarms of small, short-lived data streams characteristic of microservices in a datacenter, we generate requests/responses at loads between \todo{x and x} RPS and with inter-arrival times matching a Poisson Distribution with a minimum of \todo{x and maximum of x}. The traffic consists of data from the Github URI request dataset ~\cite{github-dataset}.

\noindent\textit{Big Pipe}
Long running single src, single dst compression/decompression
- Workload to optimize: compression/decompression of a very long data stream
	- Setup: Fixed (High) Compression ratio; compress long data stream
	- Figure of merit: CPU utilization x Runtime (or progress made on input stream)
		- Exceeding 10% CPU util incurs penalty with each % point over 10% incurring more penalty

\malian{One important, relevant design that we need to compare against is reconfiguration HW (i..e, FPGA). FPGA's area is higher than ASIC, but it offer reconfigurability. We should quantify the prose and cons of FPGA in our analysis. This work "Comparing FPGA vs. Custom CMOS and the Impact on Processor Microarchitecture" claims that FPGA area is 18~35X more than ASIC implementation. Then from silicon efficiency perspective FPGA are even worst! We should develop a first order model and compare ASIC accelerator vs. FPGA accelerator vs. general purpose cores vs. our design}
%We explore the following configurations for near-data compression units using the gem5 simulator:

%\begin{itemize}
%\item An ARM N1 Neoverse processor implemented in the Gem5 Novoverse framework.~\cite{gem5-novoverse} \malian{do we have Neoverse gem5 framework?}
%\item A in-order \malian{you mean out of order?} core with various design space parameters (L1/L2 cache, BTBs, ROBs, fetch width)  

%\end{itemize}

%On the following workloads:

%\begin{itemize}
%\item Page Compression/decompression of representative data acquired from google workload traces~\cite{hyperprotobench}
\malian{we need to be able to run various compression algorithms w/ various compression block sizes. \arch need to be able to provide speedup across all different algorithms.}
%\end{itemize}
